Progressive Transmission and Inference of Deep Learning Models

Modern image files are usually progressively transmitted and provide a preview before downloading the entire image for improved user experience to cope with a slow network connection. In this paper, with a similar goal, we propose a progressive transmission framework for deep learning models, especially to deal with the scenario where pre-trained deep learning models are transmitted from servers and executed at user devices (e.g., web browser or mobile). Our progressive transmission allows inferring approximate models in the middle of file delivery, and quickly provide an acceptable intermediate outputs. On the server-side, a deep learning model is divided and progressively transmitted to the user devices. Then, the divided pieces are progressively concatenated to construct approximate models on user devices. Experiments show that our method is computationally efficient without increasing the model size and total transmission time while preserving the model accuracy. We further demonstrate that our method can improve the user experience by providing the approximate models especially in a slow connection.

==> 6_discussion.tex <==
\section{Discussion}
\label{section:discussion}

We have introduced a simple implementation of progressive transmission of deep learning models.
However, we consider that there could be various methods to implement progressive transmission in a better way.
In this section, we introduce some of the interesting methods that can be covered in the future.
% with the hope that academia and industry are discussing these methods continually.

\subsection{Interactive Application using Progressive Models}

Unlike the images, the deep model transmission can be stopped before the entire model file is delivered.
For example, inference results from a 6-bit model and the results from a 16-bit model might be the same.
In this case, we do not have to transmit all the parts of the model.
However, it is difficult to determine when to stop transmission in the real-world since we do not know whether the result is correct or wrong.
Instead of a rule-based policy to stop the transmission, we introduce an alternative policy to delegate to the users to decide whether to continue the transmission or to stop it.

Figures \ref{fig:policy3} illustrates an example of user flow when using this policy.
In this policy, an approximate model is delivered to the user firstly, and then the rest of the model is transmitted when the user clicks the retry button.
We argue that users are already familiar with the retry button or the refresh button, and we expect this policy will not be difficult for the users.
Although this policy may make the application a little more complicated, we expect it to be effective in some cases.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/interactive_app.pdf}
    \caption{\label{fig:policy3} Example of a face detection application that progressively loads the model through user actions.}
\end{figure}


\subsection{Using the Width-Multiplier on Progressive Model Representation}

In Section \ref{section:framework_design}, we introduced a framework that divides the model based on the float precision.
In addition to using the float precision, there are many ways to design the schemes and methods for progressive transmission.
Among them, width multiplier seems to be efficient.
Slimmable networks \cite{yu2019slimmable,yu2019universally} shows that they could produce a single network that can be run in various width multipliers without any accuracy losses.
Thus, we could adopt their idea as a method for progressive transmission.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/width_multiplier.pdf}
    \caption{Imaginary design of the width-multiplier based progressive model transmission framework}
    \label{fig:width_multiplier_approach}
\end{figure}

Figure \ref{fig:width_multiplier_approach} illustrates an imaginary framework when we adopt the width-multiplier approach.
While the width multiplier method is a little more complicated to implement than the float precision method, it has an advantage that it can be applied simultaneously with quantization, which makes the model size much smaller and allows the first inference result to occur much faster.




